Non-iterative recomputation of dense layers for performance improvement of DCNN

An iterative method of learning has become a paradigm for training deep convolutional neural networks (DCNN). However, utilizing a non-iterative learning strategy can accelerate the training process of the DCNN and surprisingly such approach has been rarely explored by the deep learning (DL) community. It motivates this paper to introduce a non-iterative learning strategy that eliminates the backpropagation (BP) at the top dense or fully connected (FC) layers of DCNN, resulting in, lower training time and higher performance. The proposed method exploits the Moore-Penrose Inverse to pull back the current residual error to each FC layer, generating well-generalized features. Then using the recomputed features, i.e., the new generalized features the weights of each FC layer is computed according to the Moore-Penrose Inverse. We evaluate the proposed approach on six widely accepted object recognition benchmark datasets: Scene-15, CIFAR-10, CIFAR-100, SUN-397, Places365, and ImageNet. The experimental results show that the proposed method obtains significant improvements over 30 state-of-the-art methods. Interestingly, it also indicates that any DCNN with the proposed method can provide better performance than the same network with its original training based on BP.

==> tikzlibrarysecdia.code.tex <==
% = = = = = = = = = = = = = = = =
% Sector diagram library 7/10/2013
% = = = = = = = = = = = = = = = =
%\usepackage{pgfplots}
\usetikzlibrary{backgrounds,calc,shapes.geometric}
\pgfdeclarelayer{sector-back}
\pgfdeclarelayer{sector-middle}
\pgfsetlayers{sector-back,sector-middle,main}

\newcommand{\deflistentries}[1]{
\gdef\listentries{}% global list
\foreach \x[count=\xi] in {#1}{\global\let\maxitems\xi}% count the max number of items
\foreach \x[count=\xi] in {#1}{
 \ifnum\xi=\maxitems
   \xdef\listentries{\listentries \x}
 \else
   \xdef\listentries{\listentries \x,}
 \fi
}
}
\newcommand{\deflistcolors}[1]{
\gdef\listcolors{}% global list
\foreach \x[count=\xi] in {#1}{\global\let\maxitemcolors\xi}% count the max number of items
\foreach \x[count=\xi] in {#1}{
 \ifnum\xi=\maxitemcolors
   \xdef\listcolors{\listcolors \x}
 \else
   \xdef\listcolors{\listcolors \x,}
 \fi
}
}

% list of keys
\pgfkeys{/tikz/.cd,
  diagram angle/.store in=\refangle,
  diagram angle=30,
  diagram radius/.store in=\diagramradius,
  diagram radius=10,
  diagram step/.store in=\diagramstep,
  diagram step=1,
  diagram axes precision/.store in=\diagramprecision,
  diagram axes precision=1,
  diagram x label/.store in=\diagramxlabel,
  diagram x label={Scene15 dataset},
  diagram y label/.store in=\diagramylabel,
  diagram y label={CIFAR10 dataset},
  diagram x label pos/.store in=\diagramxlabelpos,
  diagram x label pos=135:\diagramradius,
  diagram y label pos/.store in=\diagramylabelpos,
  diagram y label pos=270:\diagramradius,
  options x label/.store in=\diagramxoptions,
  options x label={},
  options y label/.store in=\diagramyoptions,
  options y label={},
  draw axes/.code={
    \pgfmathsetmacro\diagramsecondstep{2*\diagramstep}
    \begin{pgfonlayer}{sector-back}
    \foreach \angle in {0,\refangle,...,360}{
      \draw[help lines,dashed](0,0) --++(\angle:\diagramradius);
    }
    \draw(-\diagramradius,0)--(\diagramradius,0);
    \draw(0,-\diagramradius)--(0,\diagramradius);
    \foreach \x in {\diagramstep,\diagramsecondstep,...,\diagramradius}{
      \draw[help lines,dashed](0,0) circle[radius=\x];
      \draw(\x,0.1)--(\x,-0.1);
      \draw(0.1,\x)--(-0.1,\x);
      \draw(-\x,0.1)--(-\x,-0.1);
      \draw(0.1,-\x)--(-0.1,-\x);
    }
    \end{pgfonlayer}

     \foreach \x in {\diagramstep,\diagramsecondstep,...,\diagramradius}{

      \node[fill=white,draw,inner sep=1.5pt,font=\footnotesize] at (0,\x)
      {\pgfmathprintnumber[fixed,
        precision=\diagramprecision,
        fixed zerofill,
      ]{\x}

      };
    }
    \node[fill=white,draw,inner sep=1.5pt] at (0,0){0};
    \node[fill=white,\diagramxoptions] at (\diagramxlabelpos){\diagramxlabel};
    \node[fill=white,\diagramyoptions] at (\diagramylabelpos){\diagramylabel};
  },
  sector angle/.store in=\sectorangle,
  sector angle=\refangle,
  sector color/.store in=\sectorcolor,
  sector color=green!80!black,
  sector opacity/.store in=\sectoropacity,
  sector opacity=0.8,
  sector amplitude/.store in=\sectoramplitude,
  sector amplitude=1cm,
  sector rotation/.store in=\sectorrotation,
  sector rotation=\sectorangle/2,
  sector amplitude=1,
  draw sector/.code={
    \begin{pgfonlayer}{sector-middle}
    \node[circular sector,
          draw,
          fill=\sectorcolor,
          opacity=\sectoropacity,
          circular sector angle=\sectorangle,
          anchor=sector center,
          minimum width=\sectoramplitude,
          rotate=\sectorrotation]
          at (0,0){};
    \end{pgfonlayer}
  },
  draw sector list/.code={
    \foreach \ampli/\thiscolor[count=\xi from 0] in {#1}{
            \pgfmathtruncatemacro\thisrotation{\sectorangle/2+\xi*\sectorangle}
            \sector[sector color=\thiscolor,
               sector amplitude=\ampli,
               sector rotation=\thisrotation,
               draw sector]{};
    }
  },
}

\tikzset{sector legend/.style={
  circular sector,
  draw,
  opacity=\sectoropacity
  }
}
% definition to insert numbers
\pgfkeys{/pgfplots/sector in legend/.style={%
        /pgfplots/legend image code/.code={%
            \node[sector legend,#1] at (0,0){};
        },%
    },
}

% main commands
\def\drawaxes{\tikz@path@overlay{node}}
\def\sector{\tikz@path@overlay{node}}
\def\sectorlist{\tikz@path@overlay{node}}
\def\sectorlegendimage#1{\addlegendimage{sector in legend={#1}}}
\def\legendlistcolors#1{%
\pgfplotsinvokeforeach{#1}{
\sectorlegendimage{fill=##1}}
}

% legend stuff
%%--------------------------------
% Code from Christian Feuers?nger
% https://tex.stackexchange.com/questions/54794/using-a-pgfplots-style-legend-in-a-plain-old-tikzpicture#54834

% argument #1: any options
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

%%--------------------------------

